Self-Assembly of Patterns in the abstract Tile Assembly Model

In the abstract Tile Assembly Model, self-assembling systems consisting of tiles of different colors can form structures on which colored patterns are ``painted.'' We explore the complexity, in terms of the numbers of unique tile types required, of assembling various patterns. We first demonstrate how to efficiently self-assemble a set of simple patterns, then show tight bounds on the tile type complexity of self-assembling 2-colored patterns on the surfaces of square assemblies. Finally, we demonstrate an exponential gap in tile type complexity of self-assembling an infinite series of patterns between systems restricted to one plane versus those allowed two planes.

==> results.tex <==

\section{Results}

% \subsection{Random}

% \begin{enumerate}
%     \item For the case of a 2-colored pattern, does it matter if the requirements are loosened, and the assembly doesn't have to assemble the entire square, but just the tiles of a certain color? This would mean the pattern is just some connected shape bounded in a $n \times n$ square. My gut intuition is it doesn't make it any easier because a "spiral" assembly would take $n^2$ tile types. 
% \end{enumerate}

% \subsection{1D patterns}



% Ideas:
% \begin{enumerate}
%     \item Single layers of tile growth in 1D behave like finite-state transducers (DFAs which output a symbol during each transition).


%     \item What is the tile complexity of assembling a $1 \times n$ pattern (it seems trivial that it should be n tile types) 

%     \item What is the tile complexity of assembling a $1 \times n$ pattern in a given area but the assembly can grow anywhere in the 2d plane? (I bet it is a small overhead on Kolmogorov complexity of the pattern.)

%     \item What is the tile complexity of assembling a $1 \times n$ pattern when the assembly is bounded to a $2 \times n$ rectangle? 

%     \item The canonical representation of an RE language, i.e. $f(n) = n$, cannot weakly self-assemble (see \cite{jCCSA}). Scott and I think that perhaps we can prove a lower bound of $n\log(n)$. The upper bound in \cite{jCCSA} of $n^2$ seems solid and impossible (using known techniques at least) to bring down. Can we bring the lower bound up to match that?
    
% \end{enumerate}

(Obsolete) Ideas:
\begin{enumerate}
    \item Given an arbitrary (2-colored) pattern contained within an $n \times n$ square, an information theoretic argument should (probably) hold that there exist such patterns that require $O(n^2/\log(n))$ tile types since there exist strings of length $n^2$ that are incompressible and each tile type contains $\log(n^2) = O(\log(n))$ bits. We have a construction that can weakly self-assemble any pattern on an $n \times n$ square using $O(n^2/\log(n))$ tile types. Tight. The construction works by hard-coding a ``comb'' where the ``teeth'' of the comb are $\log(n)$ locations apart. Then, a set of $n$ tile types are used as ``fillers'' to attach to the teeth and fill in the gaps with the necessary patterns (since there will be exactly one combo of filler tiles for each possible pattern of length $\log(n)$.
    
    \item How does the tile complexity of building $n\times n$ squares increase if we require a regular $k\times k$ grid pattern of glues to protrude from the square's surface? We can still probably beat $O(n^2)$ by a large margin, maybe $O(\log(n)\log(k))$?

    \item What minimum tile complexity is needed to build an $n \times n$ pattern in a designated area? The assembly can grow anywhere in a 2D plane. 
 
    \item How does the complexity of assembling a pattern compare to assembling that pattern tessellated across the whole plane? 
 
    \item How complex is it to assemble a pattern that is all the same color except a single tile(black)? How can you add more black tiles to the pattern so the complexity scales somewhat linearly? How many black tiles can there be before this skyrockets to $n^2$?

    \item What is the tile complexity of assembling a $n \times n$ pattern that contains a single horizontal or vertical line? 

    \item How about when there can be any number of lines in the pattern?

    \item What is the tile complexity of assembling a $n \times n$ pattern that contains a diagonal line? With different slopes? 
    
\end{enumerate}


%     \subsection{Scott's stuff}

% \begin{enumerate}
%     \item Let $w$ be an $n$-bit binary string and $c < n$.

%     \item Then, the number of strings of length less than $n-c$ is $1+2+4+ ... + 2^{n-c-1} = 2^{n-c}-1 < 2^{n-c}$.

%     \item Let $e > 0$ be a fixed, real constant, and define the set  $A_e = \{ w \mid K(w) >= |w|-e|w| = (1-e)|w| \}$.

%     \item Then, $|A_e| / |\{0,1\}^n| = ((2^{|w|} - 2^{|w|-e|w|})+1) / 2^{|w|} > 1 - (1/2)^{e|w|}$, which basically means that the fraction of $n$-bit strings having the property that $K(w) >= (1-e)|w|$ tends to $1$ as $n$ goes to infinity. 

%     \item In other words, $A_e$ has density $1$, which I believe is what is meant by the statement ``$K(w) >= (1-e)|w|$ for almost all strings $w$.''
% \end{enumerate}



